FlowTune: End-to-end Automatic Logic Optimization Exploration via Domain-specific Multi-armed Bandit

Recent years have seen increasing employment of decision intelligence in electronic design automation (EDA), which aims to reduce the manual efforts and boost the design closure process in modern toolflows. However, existing approaches either require a large number of labeled data and expensive training efforts, or are limited in practical EDA toolflow integration due to computation overhead. This paper presents a generic end-to-end sequential decision making framework FlowTune for synthesis tooflow optimization, with a novel high-performance domain-specific, multi-stage multi-armed bandit (MAB) approach. This framework addresses optimization problems on Boolean optimization problems such as a) And-Inv-Graphs (# nodes), b) Conjunction Normal Form (CNF) minimization (# clauses) for Boolean Satisfiability; logic synthesis and technology mapping problems such as c) post static timing analysis (STA) delay and area optimization for standard-cell technology mapping, and d) FPGA technology mapping for 6-in LUT architectures. Moreover, we demonstrate the high extnsibility and generalizability of the proposed domain-specific MAB approach with end-to-end FPGA design flow, evaluated at post-routing stage, with two different FPGA backend tools (OpenFPGA and VPR) and two different logic synthesis representations (AIGs and MIGs). FlowTune is fully integrated with ABC [1], Yosys [2], VTR [3], LSOracle [4], OpenFPGA [5], and industrial tools, and is released publicly. The experimental results conducted on various design stages in the flow all demonstrate that our framework outperforms both hand-crafted flows [1] and ML explored flows [6], [7] in quality of results, and is orders of magnitude faster compared to ML-based approaches.

==> TCAD21-FlowTune/figs/result_aig.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\caption{\textit{FTune} in AIG minimization (minimizing the number of AIG nodes). \texttt{Best-base} is the best baseline result obtained from hand-crafted scripts and ML-based approaches \cite{DBLP:conf/dac/YuXM18,hosny2019drills}; $s$:$m$ (e.g., 2:30) shows the \# stages verses \# iterations per stage.}
\vspace{-3mm}
\label{fig:result_aig}
\end{figure*}


==> TCAD21-FlowTune/figs/result_cnf.tex <==
\begin{figure}[!htb]
\centering
% inputs
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_1.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_2.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_3.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\caption{CNF Clauses minimization}
\vspace{-3mm}
\label{fig:result_cnf}
\end{figure}


==> TCAD21-FlowTune/figs/result_fpga.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\caption{\textit{FTune} in LUT minimization for FPGA technology (6-in LUT devices). \texttt{Best-base} is the best baseline result obtained from hand-crafted scripts and ML-based approaches \cite{DBLP:conf/dac/YuXM18,hosny2019drills}; $s$:$m$ (e.g., 2:30) shows the \# stages verses \# iterations per stage.}
\label{fig:result_fpga}
\end{figure*}


==> TCAD21-FlowTune/figs/result_std.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_3.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_9.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\caption{Timing closure STD cell mapping with gate sizing, post STA.}
\label{fig:result_std}
\end{figure*}


==> abstract.tex <==
\begin{abstract}

Design flows are the explicit combinations of design transformations, primarily involved in synthesis, placement and routing processes, to accomplish the design of Integrated Circuits (ICs) and System-on-Chip (SoC). Mostly, the flows are developed based on the knowledge of the experts. However, due to the large search space of design flows and the increasing design complexity, developing \textit{Intellectual Property (IP)-specific} synthesis flows providing high Quality of Result (QoR) is extremely challenging. This work presents a fully autonomous framework that artificially produces design-specific synthesis flows without human guidance and baseline flows, using Convolutional Neural Network (CNN). The demonstrations are made by successfully designing logic synthesis flows of three large scaled designs.

\end{abstract}

==> figs/result_aig.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/aig_opt_plots/aig_target_0_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\caption{\textit{FTune} in AIG minimization (minimizing the number of AIG nodes). \texttt{Best-base} is the best baseline result obtained from hand-crafted scripts and ML-based approaches \cite{DBLP:conf/dac/YuXM18,hosny2019drills}; $s$:$m$ (e.g., 2:30) shows the \# stages verses \# iterations per stage.}
\vspace{-3mm}
\label{fig:result_aig}
\end{figure*}


==> figs/result_cnf.tex <==
\begin{figure}[!htb]
\centering
% inputs
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_1.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_2.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.22\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/cnf_opt_plots/bmc_3.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\caption{CNF Clauses minimization}
\vspace{-3mm}
\label{fig:result_cnf}
\end{figure}


==> figs/result_fpga.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\begin{minipage}{0.32\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/fpga_opt_plots/fpga_target_4_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\caption{\textit{FTune} in LUT minimization for FPGA technology (6-in LUT devices). \texttt{Best-base} is the best baseline result obtained from hand-crafted scripts and ML-based approaches \cite{DBLP:conf/dac/YuXM18,hosny2019drills}; $s$:$m$ (e.g., 2:30) shows the \# stages verses \# iterations per stage.}
\label{fig:result_fpga}
\end{figure*}


==> figs/result_std.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_3.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_9.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\hspace{0.5mm}
\begin{minipage}{0.23\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\caption{Timing closure STD cell mapping with gate sizing, post STA.}
\label{fig:result_std}
\end{figure*}


==> figs/result_std_area.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_3_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_3_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_3_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_3_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_3_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_3_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\vspace{-3mm}
\caption{\textit{FTune} in area optimization using gate sizing. QoR results are obtained using Genus with ASAP 7nm library.}
\label{fig:result_std_area}
\end{figure*}


==> figs/result_std_delay.tex <==
\begin{figure*}[!htb]
\centering
% inputs
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_4.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_5.pdf}
%\subcaption{Input3}\label{fig:input3}
\end{minipage}
%
\hspace{0mm}
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_6.pdf}
%\subcaption{Input4}\label{fig:input4}
\end{minipage}
% outputs
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_7.pdf}
%\subcaption{Output1}\label{fig:Output1}
\end{minipage}
\begin{minipage}{0.3\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/std_map_plots/std_target_2_11.pdf}
%\subcaption{Output2}\label{fig:Output2}
\end{minipage}
%
\vspace{-3mm}
\caption{\textit{FTune} in STA delay optimization with gate sizing. QoR results are obtained using Genus with ASAP 7nm library.}
\label{fig:result_std_delay}
\end{figure*}


==> preamble/authorlist.tex <==
\newbool{journalBasedAuthors}
\ifCLASSOPTIONpeerreview \setbool{journalBasedAuthors}{true}
\else \ifCLASSOPTIONjournal \setbool{journalBasedAuthors}{true}
\else \setbool{journalBasedAuthors}{false}
\fi
\fi

\ifbool{journalBasedAuthors}
{

    \author{Walter~Lau Neto, 
            Yingjie~Li,
            Pierre-Emmanuel~Gaillardon, 
            Cunxi~Yu
    %\thanks{Manuscript received April XX, 2016; revised Month DD, 2016.}%
    \thanks{W. Lau Neto is with Silicon Realization Group of Synopsys Inc., Sunnyvale, CA, US. (e-mail: launeto@synopsys.com).}
    \thanks{Y. Li, P-E. Gaillardon, and C. Yu are with the Department of Electrical and Computer Engineering, University of Utah, Salt Lake City, US (e-mails: yingjie.li@utah.edu, pierre-emmanuel.gaillardon@utah.edu, cunxi.yu@utah.edu).}
    \thanks{This work is funded by National Science Foundation (NSF) NSF-2008144, DARPA IDEA, and NSF CAREER awards NSF-1751064 and NSF-2047176.}
    \ifCLASSOPTIONjournal
        \thanks{Digital Object Identifier 10.1109/TCAD.XXXXXXX}
    \fi
    }
}





==> related-ml4syn.tex <==
%\section{Approach}
\section{Related Work}

Recently, we have seen significant progress in leveraging ML techniques for logic synthesis. Specifically for exploring synthesis flows as sequential decision making problem, there are mainly two directions -- (1) learning a static ML-based predictor to enable fast design space and (2) exploring flows in reinforcement and iterative fashion. 

In \cite{DBLP:conf/dac/YuXM18}, Yu et al. proposed the first ML-based flow exploration approach, which involves a CNN-based QoR predictor to enable fast flow exploration and generation. They model the problem as a multi-class classification problem, and the CNN outputs angel- and devil-flows, where angel flows produce the best QoR results and devil flows likely offers the worst QoR. While this approach learns a static ML model that eliminates the expensive runtime of evaluating a large number of flows in synthesis tool, one critical drawback is on the data collecting and labelling. Although, the authors proposed a follow-up approach based on recurrent neural networks and transfer learning to reduce the efforts in collecting labelled dataset, this approach is limited on limited technology domain, which is limited on generalizability for technology transferability \cite{yu2020decision}.

{To work around the challenge of labelled data collection, reinforcement learning (RL) approaches has then been adopted for logic synthesis flow generation}. Liu et. al. \cite{liu2017parallelized} first cast logic optimization as a \textit{Markov Decision Process} (MDP), where a set of logic transformations could be chosen in the next iteration of the synthesis flow. However, it has been demonstrated that the performance of a sequence of logic synthesis transformations does not satisfy MDP properties, since the performance of each transformation does not solely depend on previous transformation.  Hosny et al. \cite{hosny2019drills} propose a Deep RL-based approach that aims to optimize the area given a timing constraint. They cast the generation of logic synthesis flow into a game-like problem, where the actions are the set of transformations to be selected. However, the RL training process is very time consuming and offers poor flexibility (e.g., limited flow lenghth, QoR-specific RL model, etc.,) and integration capability. %The generated flows do not have fixed length and may vary on the number of transformations to apply. Results show the effectiveness of the agent to optimize area while respecting the delay constraint. 

%Another important observation is that this work considers each transformation to happen a same fixed amount of times $m$. Thus, \cite{DBLP:conf/dac/YuXM18} limits the theoretical search space of flow exploration to a multi-set permutation problem. While this work was one of the firsts to apply ML for autonomous flow generation, many others followed this direction by applying reinforcement-learning and Graph Neural Networks (GNNs), as depicted in the next Sections. 

%Other static approaches on ML for logic synthesis are applied into different tasks, such as choosing an appropriate logic representation for circuit partitions \cite{lso}, predicting critical paths \cite{easyopt}, and cut-pruning for technology mapping \cite{slap}. 


%\subsection{Reinforcement Learning based Flow Tuning} 



%Other RL-based approaches have been used in different tasks during logic synthesis, such as approximated logic synthesis \cite{pasandi}, and gate-sizing \cite{rlsizing}. 

%\subsection{Graph Neural Networks}

To further ehance the structure information in the ML-based approaches for flow exploration, there have recently seen many works leveraging Graph Neural Network (GNNs) to improve the generalizability. Zhu et. al \cite{panrl} propose to model the logic synthesis flow generation as MDP problem and use GNNs to enhance the state representation. Therefore, besides AIG statistics and the history of transforms applied, they also aggregate the graph-structure through GNNs. They present improvements over the ABC \textit{resyn2} flow, with the same length of transformations to be applied. Similarly, in \cite{huaweirl}, the authors combine RL and GNN to optimize MIGs. In addition to utilize the feature extraction capability of GNNs, Wu \cite{wu2022hybrid} et. al. demonstrates that GNNs can be used to aggregate structure features such that static ML approaches can be trained with significantly reduced labeled data. Unfortunately, these work are only evaluated at the stage of logic-level without considering the impacts of low-level design stages such as placement and routing. % presented only for small circuits, and (ii) it compares MIGs against AIG as baselines. As MIGs are a superset of AIGs, it is expected that MIGs can represent a given circuit with fewer nodes. 

%The authors of \cite{peruvemba2021rl} present a runtime-constrained RL approach for flow generation, that also employs GNNs. In a similar way to \cite{panrl}, the authors use GNNs to represent the graph structure and take it into account as a state representation. However, opposing to \cite{panrl}, the reward function and exit condition in this case are based on the runtime constraint. The action space is given by possible transformations. The authors also consider MIGs, but with a very restricted number of transformations, i.e., only two. Compared to \cite{panrl}, the authors show they work can generate scripts that improve results in shorter runtime. Still, the authors limit their scope to a subset of small circuits from the EPFL benchamrk suite. 

%\subsection{Methods for Experimental Evaluation} 

%When designing ML models for logic synthesis, one needs to assess the trade-off between runtime overhead and accuracy of prediction. In \cite{ustun2019lamda}, the authors discuss this trade-off, showing that making QoR predictions at early stages of the flow, i.e., logic synthesis, one can achieve up to $230\times$ speedup compared to the baseline, at the price of accuracy loss. On the other hand, using pre-routing information enhances the model accuracy, but limits the speed-up gains to up to $5\times$. To balance this trade-off, the authors propose a multi-stage auto-tuning framework targeting FPGAs, leveraging online training. The authors show that their approach achieves faster design closure compared to the state-of-the-art, achieving a $5.43\times$ speed-up when comparing to an industrial auto-tuning targeting FPGAs. 


 


\section{Conclusion}


This work proposes a multi-stage multi-armed bandit framework for Boolean logic optimization that is general end-to-end and high-performance domain-specific. We present an MAB-based synthesis flow exploration technique that takes advantage of domain-specific knowledge of DAG-aware synthesis algorithms. To highlight the value of the collected domain information, a complete analysis of DAG-aware algorithms in synthesis flows is offered. We also present a novel MAB mechanism, which includes a rapid startup and a multi-stage MAB exploration strategy. We built a complete exploration framework that interfaces with numerous tools to illustrate the performance and versatility of our framework. Our results show that FlowTune outperforms prior works in terms of optimization efficiency and runtime for standard-cell technology mapping, as well as end-to-end PnR assessment using various backend tools. This is the first framework that shows end-to-end synthesis experiments in terms of post-PnR performance indicators. We also show that our domain-specific MAB algorithm can be applied to a variety of DAG-based logic synthesis, with FlowTune being used for both AIG and MIG improvements. Explainability and robustness analysis of ML-based design space exploration, as well as architecture-aware optimizations will be the focus of future work.


\textbf{Acknowledgement} This work is funded by National Science Foundation (NSF) NSF-2008144, DARPA IDEA, and NSF CAREER awards NSF-1751064 and NSF-2047176.



==> results-flowtune.tex <==
\section{Experimental Results}\label{sec:result}
 

The experimental results are obtained using a CentOS 7 machine with a 48-core Intel Xeon operating at 2.1 GHz, 8 TB RAM, and 2 TB SSD. We demonstrate the proposed approach using six designs obtained from VTR 8.0 \cite{luu2014vtr}. FlowTune offers high flexibility and effectiveness in optimizing the logic synthesis procedures. Thus, we present results for different scenarios, from technology independent optimization to post mapping results for ASIC, and post-PnR results for FPGA. 
%In particular, we present results for AIG minimization, standard cell technology mapping, post-PnR evaluation with Xilinx Vivado, post-PnR evaluation with VTR 8.0, 
Particularly, in this work, we focus on end-to-end design scenarios to demonstrate the effectiveness at post-PnR stage, including post-PnR assessment of AIGs + VPR flow and MIGs + OpenFPGA flow. Table \ref{tbl:benchmark} summarizes the number of I/O pins, the number of nodes, the logic depth, and a number of latches of the selected benchmarks. In both cases, i.e., when we consider VTR flow with AIG, or MIG-based flow for OpenFPGA, the number of initial nodes are the same. {Note that all synthesis transformations for MIG and AIG flows are all remaining unchanged w.r.t their original implementations.} 

\begin{table}[h]
\centering
\caption{Details of selected VTR benchmarks for evaluating FlowTune. The designs are converted into BLIF format using VTR flow.}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Design} & \textbf{I/O} & \textbf{Nodes} & \textbf{Latch} & \textbf{Level} \\ \hline
\textit{bfly} & 482/257 & 28910 & 1748 & 97 \\ \hline
\textit{dscg} & 418/257 & 28252 & 1618 & 92 \\ \hline
\textit{fir} & 450/225 & 27704 & 1882 & 94 \\ \hline
\textit{ode} & 275/169 & 16069 & 1316 & 98 \\ \hline
\textit{or1200} & 588/509 & 12833 & 670 & 148 \\ \hline
\textit{syn2} & 450/321 & 30003 & 1512 & 93 \\ \hline
\end{tabular}
\label{tbl:benchmark}
\end{table}


 
\subsection{Standard Cell Technology Mapping}\label{sec:result:std}

It is known that technology-independent metrics have often miss-correlation with post-technology mapping results \cite{liu2017parallelized}. Yet, many logic synthesis works limit the results and analysis to node count and logic depth, instead of actual post-mapping area and delay. In this work, we aim to show that \textit{FlowTune} can find good solutions post-mapping, and is not limited to DAG size and depth reduction. With this experiment, we show that \textit{FlowTune} is portable and easy to integrate, besides improving the desing post-mapping, which is ubiquitous to make this approach practical.

\textbf{STD technology mapping optimization with FlowTune}: We aim to optimize the technology-mapping QoR, evaluated by Cadence Genus {with gate sizing}, using the ASAP 7nm library, while targeting \textbf{a)} STA delay optimization (Figure \ref{fig:result_std_delay}); and \textbf{b)} area optimization (Figure \ref{fig:result_std_area}). QoR results are collected with Genus by importing the mapped Verilog from ABC. To the best of our knowledge, this is the first work that addresses synthesis flow tuning for STA-aware technology mapping. 

We can see that \textit{FlowTune} effectively explores the design space by finding better synthesis flows for both area and post-STA delay optimization. However, \textit{FlowTune} is not able to find any better synthesis flow after the initialization for design \texttt{or1200}. This is similar to what we observed during the FPGA experiments for this same design \ref{fig:vpr_area}. We believe the ABC synthesis flow design space of \texttt{or1200} is very limited. While for delay different \textit{FlowTune} setups perform better in different designs, for area a setup ($s:m$ = 2:30) performs consistently better than others. Thus, while targeting area optimization, \textit{FlowTune} can be set with $s:m$ = 2:30. {The runtime cost of FlowTune of all benchmarks listed in Table \ref{tbl:benchmark} vary from 433 seconds to 1104 seconds, with average 892 seconds runtime cost, as depicted in Table IV, for AIG optimization. Note that the runtime overhead of FlowTune is the same regardless if used with AIGs or MIGs. Thus, the overhead should be constant regardless the DAG, and runtime differences are due to the optimization for the different DAGs. Also, for larger designs partitioning could be used to run FlowTune in parallel and reduce the runtime.  }


\begin{table}[t]

\centering
 {\caption{FlowTune runtime for synthesis exploration for AIGs.}}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|clllll|}
\hline
\multirow{2}{*}{} &
  \multicolumn{6}{c|}{\textbf{Design}} \\ \cline{2-7} 
 &
  \multicolumn{1}{c|}{\textit{bfly}} &
  \multicolumn{1}{c|}{\textit{dscg}} &
  \multicolumn{1}{c|}{\textit{fir}} &
  \multicolumn{1}{c|}{\textit{ode}} &
  \multicolumn{1}{c|}{\textit{or1200}} &
  \multicolumn{1}{c|}{\textit{syn2}} \\ \hline
\textbf{Runtime(s)} &
  \multicolumn{1}{l|}{1,101.94} &
  \multicolumn{1}{l|}{1,052.88} &
  \multicolumn{1}{l|}{1,049.94} &
  \multicolumn{1}{l|}{611.96} &
  \multicolumn{1}{l|}{433.93} &
  1,104.80 \\ \hline
\end{tabular}%
}
\end{table}

%, we are not able to derive a setup that likely will perform better than others for standard-cell mapping delay optimization. However, for standard-cell area minimization, we observe the a similar result as for AIG and LUT minimization, such that a similar setup would likely benefit standard-cell mapping area. %While these observations offer some intuition for configuring \textit{FlowTune} for different optimization objectives, we cannot provide formal explainability at this moment.



\input{TCAD21-FlowTune/figs/result_std_delay.tex}
\input{TCAD21-FlowTune/figs/result_std_area.tex}
 


\iffalse
\subsection{Case study in Vivado Flow}\label{sec:result:vivado}

%Finally, we evaluate FlowTune in an end-to-end industrial FPGA design flow (Figure \ref{fig:xilinx}). 

\begin{figure}[ht]
\centering
% inputs
\begin{minipage}{0.234\textwidth}
 \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/xilinx/xilinx_0.pdf}
%\subcaption{Input1}\label{fig:input1}
\end{minipage}
%
%\hspace{0.5mm}
\begin{minipage}{0.234\textwidth}
 \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/data/xilinx/xilinx_1.pdf}
%\subcaption{Input2}\label{fig:input2}
\end{minipage}
%
\caption{\textit{FlowTune} case studies in Vivado using two pipelined matrix multipliers generated by Vivado HLS compiler. Timing results are collected at the post-PnR stage, including logic delay and routing delay, where we observe that FlowTune improves the timing of both designs by $\sim$14\%.}
%\vspace{-5mm}
\label{fig:xilinx}
\end{figure}

For the industrial end-to-end FPGA design flow, we adopt Vivado. The input designs are two simple pipelined matrix multiplier designs generated using Vivado HLS. The baseline results are generated by running a complete design flow, i.e., Vivado HLS $\rightarrow$ Vivado. FlowTune results are generated as follows: 1) import Verilog generated by Vivado HLS into Yosys; 2) use the ABC interface in Yosys to call FlowTune for flow exploration; 3) produce Verilog using Yosys; 4) load Yosys Verilog and execute the rest of design flow using Vivado. In this integrated flow, the iterative FlowTune optimization process does not use information from PnR to minimize the runtime overhead in the original Vivado flow. Using post-PnR information is possible, given an extra runtime budget. Therefore, our integrated FlowTune has a marginal runtime overhead compared to the reference Vivado flow.
%such that the runtime overhead is marginal compared to the original Vivado flow (major runtime comes from PnR). 
\textbf{Note that we aim to show that FlowTune can benefit Vivado, and not that FlowTune can outperform/replace Vivado}. Specifically, all the results in Figure \ref{fig:xilinx} are generated without using any Xilinx IP (i.e., designs are implemented using LUTs only). There are two observations: First, we can see that FlowTune can improve $\sim$14\% post-PnR delay of both designs compared to stand-alone Vivado flow. Second, an interesting observation is that the delay distributions are significantly changed. As the technologies and FPGA architectures advance, the timing of post-PnR FPGA design is now dominated by routing delay. While using Vivado stand-alone flow, we can see that the routing delay dominates (right figures in Figure \ref{fig:xilinx}). However, we observe a significant delay distribution (logic delay vs. routing delay) changes that by using FlowTune (with ABC FPGA mapper), i.e., logic delay and routing delay are almost equivalently distributed. One possible reason is that Vivado synthesis flow has features that are PnR aware, which intends to reduce routing delay for large-scale complex FPGA designs. In contrast, the FlowTune setup in this case study only focuses on Boolean logic optimizations. %However, we do not have access to the algorithms of the industrial tool.
\fi


% \subsection{CNF Simplification}\label{sec:result:cnf}

% \textbf{Objective for FlowTune}: Minimize the number of clauses in the CNF formula generated for Bounded Model Checking (BMC) with five time frames (Figure \ref{fig:result_cnf}). \textbf{Baseline}: We compare FlowTune to the BMC simplification technique implemented in ABC, namely \texttt{dframes}. The results in Figure \ref{fig:result_cnf} are generated using \textit{3:20} setup for FlowTune. For the given four BMC instances, we can see that FlowTune achieves an average reduction of 21\% in the number of clauses. 

% \input{TCAD21-FlowTune/figs/result_cnf.tex}
% {\color{red}Walter: should we keep CNF results? it seems a bit off to me as other results are FPGA/ASIC optimizations, we could maybe just mention that during the paper and ref the ICCAD paper.}

\subsection{End-to-End Integration and Evaluation for FPGA Design}

One of the greatest challenges of leveraging ML techniques in design flow optimization is to demonstrate the optimizations can be fully realized in an end-to-end design process, e.g., evaluating the QoR performance at the post-routing stage. Therefore, in this section, we evaluate \textit{FlowTune} in two different end-to-end FPGA design frameworks, VTR 8.0 \cite{luu2011vpr} and OpenFPGA \cite{tang2019openfpga}, where our framework is integrated at the logic synthesis stage in both frameworks, for AIG and MIG. With this experiment, we aim to show the flexibility and portability of \textit{FlowTune}, along with its capabilities to improve QoR. Thus, note that our goal is not to compare VTR and OpenFPGA, or AIGs and MIGs.

\noindent
\textbf{Evaluation metrics} -- To comprehensively evaluate the FPGA implementation performance, a list of QoR metrics that cover the area (utilization) and timing are selected. Specifically, our experimental results are conducted on measuring the post-routing (a) \textit{total wirelength} (WL), (b) \textit{total area} (Area) including logic area and routing area, (c) critical path delay, and (d) total negative slack (TNS). 

\noindent
\textbf{Evaluation baselines} -- The baseline results for VTR 8.0 are generated with the default settings collected from the VTR repository. Regarding the OpenFPGA framework, we integrate \textit{FlowTune} in LSOracle, a state-of-the-art logic optimizer that handles MIG and AIGs. We focus on the MIG manipulation, and compare \textit{FlowTune} against a high-effort MIG flow in LSOracle. OpenFPGA is used with its default settings. { Besides the use of well stablished flows for AIG and MIG optimization, we have considered the use of random sampling to see how our approach compares to it. Given a timing budget of 30 minutes (which exceeds our greatest runtime), random sampling could explore $\approx$ 70 flows for \textit{bfly} on ABC, and all these flows presented worst QoR than our framework. Thus, we consider random sampling to not be a strong baseline, and adopt well-stablished design flows to be our baseline}.
Both experiments target a Stratix IV-like FPGA architecture, which is common adopted modern architecture for FPGA works \cite{gore2021scalable, luu2011vpr}. In this context, each logic block is composed of 10 fracturable LUTs, and 200 routing tracks (channels). 

\noindent
\textbf{Experimental setup for VTR 8.0 as backend} -- The experimental results conducted with VTR 8.0 as complete design flow involves the complete design flow from ODIN synthesis, with behavior Verilog HDL as inputs. The rest of the design flow includes logic synthesis and LUT-based technology mapping using ABC \cite{mishchenko2010abc}, in which \textit{FlowTune} is plugged-in to optimize the design with automatically explored design flows. The output design will then be placed and routed w.r.t to the given FPGA architecture using VPR default settings. The results included in this section are all collected at the post-routing stage. 

\noindent
\textbf{{Experimental setup for OpenFPGA as backend}} -- The OpenFPGA design flow also includes the complete design flow from ODIN synthesis, with behavior Verilog HDL as inputs. Then it uses LSOracle to read an input BLIF into a MIG, and perform logic optimization. \textit{FlowTune} is integrated with LSOracle to autonomously generate a MIG-based flow. LSOracle is then used for LUT mapping, and the output is dumped into a BLIF file. The BLIF is then used as input to OpenFPGA with default settings, and all the results are collected post-routing. {Note that LSOracle synthesis framework is MIG-based logic synthesis engine, where the transformations are all based on MIG. These experiments aim to demonstrate the DAG-based synthesis domain-specific knowledge extracted from AIG optimization is transferable to MIG as well.}

To show the flexibility of our approach, we present results for two different end-to-end FPGA design evaluations, i.e., FlowTune in VTR 8.0 and FlowTune in LSOracle + OpenFPGA. Note that we do not intend to compare the differences between logic synthesis data structures (i.e., AIG and MIG), and do not intend to compare the performance across different backend frameworks (VTR and OpenFPGA). In summary, our goal with these experiments is to show that FlowTune can be easily integrated and verify its effectiveness in different scenarios. 


\begin{figure*}[t]
\centering
% inputs
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/VTR_results/Area_VTR.pdf}
\subcaption{Total logic and routing area.}\label{fig:vpr_area}
\end{minipage}
%
\hspace{5mm}
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/VTR_results/Total_Wirelength_VTR.pdf}
\subcaption{Total routing wirelength.}\label{fig:vpr_wl}
\end{minipage}
%
\\
\hspace{0mm}
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/VTR_results/TNS_VTR.pdf}
\subcaption{Post-PnR total negative slacks (TNS).}\label{fig:vpr_tns}
\end{minipage}
\hspace{5mm}
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/VTR_results/WNS_VTR.pdf}
\subcaption{ Post-PnR critical path delay.}\label{fig:vpr_delay}
\end{minipage}
\caption{ Post-routing evaluation with VTR (VPR PnR) as backend using six benchmarks collected from \cite{luu2014vtr}, with default VTR 8.0 flow as baseline where logic synthesis is conducted on \textbf{AIG logic optimization}. The collected results include (a) total area including logic and routing area, (b) total routing wire length, (c) post-PnR total negative slacks (TNS), and (d) post-PnR critical path delay.}
\label{fig:result_vpr}
\end{figure*}

\begin{figure*}[t]
\centering
% inputs
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/OFPGA-MIG/Area.pdf}
\subcaption{Total logic and routing area.}\label{fig:ofpga_area}
\end{minipage}
%
\hspace{5mm}
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/OFPGA-MIG/Wirelength.pdf}
\subcaption{Total routing wirelength.}\label{fig:ofpga_wl}
\end{minipage}
%
\\
\hspace{0mm}
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/OFPGA-MIG/TNS.pdf}
\subcaption{Post-PnR total negative slacks (TNS).}\label{fig:ofpga_tns}
\end{minipage}
\hspace{5mm}
\begin{minipage}{0.37\textwidth}
  \centering
\includegraphics[width=1\textwidth]{TCAD21-FlowTune/figs/OFPGA-MIG/WNS.pdf}
\subcaption{ Post-PnR critical path delay.}\label{fig:ofpga_delay}
\end{minipage}
\caption{ Post-routing evaluation with LSOracle+OpenFPGA where the logic synthesis process involves \textbf{MIG logic optimization}, with OpenFPGA as backend using the same benchmarks collected from \cite{luu2014vtr}. The results are compared to default LSOracle+OpenFPGA flow, including (a) total area including logic and routing area, (b) total routing wire length, (c) post-PnR total negative slacks (TNS), and (d) post-PnR critical path delay.}
\label{fig:result_ofpga}
\end{figure*}

\medskip
\noindent
\textbf{Results on total area} -- (1) \textbf{VTR results} -- Figure \ref{fig:vpr_area} shows the results of post-routing evaluation on design area which is the sum of total used logic block area and the total routing area. When designs are evaluated with \textit{FlowTune}, the area can be reduced by $\sim30\%$ on average for \texttt{bfly}, \texttt{dscg}, \texttt{fir}, \texttt{ode}, and \texttt{syn2}. %The improvements can be comparable or even better when the designs are optimized with reduced \textit{FlowTune} efforts. Specifically, for design \texttt{bfly}, the area can be further optimized with implemented with reduced \textit{FlowTune}. 
However, for design \texttt{or1200}, we can achieve few improvement results with \textit{FlowTune} optimization. (2) \textbf{OpenFPGA results} -- OpenFPGA results show area improvements in all the cases, as seen in Figure  \ref{fig:ofpga_area}. Results present up to 10.0\% area improvement, with an average of 4.5\% area reduction. While these results are not as expressive as in the VTR flow, it is still relevant and consistent among both flows. 

\medskip
\noindent
\textbf{Results on total wirelength} -- (1) \textbf{VTR results} -- We further analyze the total wirelength of the post-PnR designs to clearly show that routing has been improved, in addition to the logic optimization results. Figure \ref{fig:vpr_wl} shows the results of post-routing evaluation on total routing wirelength. The performance with \textit{FlowTune} can be improved for all designs. %Also, the results show that reduced \textit{FlowTune} will lead to reduced optimization with some degradation. However, compared to the savings in runtime, the performance of reduced \textit{FlowTune} can be worth it depending on the application. 
Similarly, for total area evaluation, the improvement is marginal for design \texttt{or1200}. (2) \textbf{OpenFPGA results} -- Figure  \ref{fig:ofpga_wl} presents the total wirelength for MIGs with OpenFPGA. In this case, \textit{FlowTune} presents better results in 4 cases, with little overhead in two designs (up to 4\%). On the other hand, \textit{FlowTune} reduces the total wirelength in up to 14\%, and 5\% on average. As the goal of \textit{FlowTune} is to reduce the logic area, it might reflect in longer total wirelength in some cases due to the improved logic sharing. Still, the overhead compared to the baseline flow was small for the considered designs. We can observe that \textit{FlowTune} was able to consistently reduce total wirelength in both flows for almost all the benchmarks. When considering \texttt{or1200}, in the VTR flow, \textit{FlowTune} had minor gains compared to the baseline, whereas in OpenFPGA it had some overhead compared to the baseline. 
%Therefore, \texttt{or1200} shows to be a case where 


\medskip
\noindent
\textbf{Results on timing} -- Post-PnR timing results are presented with critcal path delay and total negative slacks (TNS), which are the most critical two metrics used for timing evaluation. (1) \textbf{VTR results} -- The performance with \textit{FlowTune} can be improved for all designs except for \texttt{or1200}. %Additionally, for the critical path delay, the reduced \textit{FlowTune} can even perform better for all designs. Specifically, design \texttt{fir} and design \texttt{ode} present greater improvements with the reducet \textit{FlowTune}. 
On the other hand, we have observed that the \texttt{or1200} timing performance has a slight improvement for TNS but got worse than the default in critical path delay. While there has been very little logic reduction (see Figure \ref{fig:vpr_area}) and wirelength reductions, the structure of the \texttt{or1200} design remains almost the same. We believe that the critical path delay and TNS results differences between with and w/o \textit{FlowTune} is from the randomness of the placement and routing algorithms in VPR. %(2) VTR results for TNS: Figure \ref{fig:vpr_tns} shows the results of post-routing evaluation on the total negative in the design. The performance of all designs can be improved with full \textit{FlowTune} implemented. For all four designs except for \texttt{or1200} and \texttt{fir}, the reduced \textit{FlowTune} can perform better than the full \textit{FlowTune} while for \texttt{or1200} and \texttt{fir}, the reduced \textit{FlowTune} perform a little bit worse than the full \textit{FlowTune} but still improve the performance compared to the baseline flow.
(2) \textbf{OpenFPGA results} -- {Figure  \ref{fig:ofpga_delay} presents the post-PnR critical path delay for the considered benchmarks.} We can see that \textit{FlowTune} greatly improves the baseline. In particular, we improve all the cases, with up to 37\% gains for the \textit{or1200}. Still, five designs have over 7\% gains in the WNS, showing the effectiveness of \textit{FlowTune} in improving MIGs over a state-of-the-art recipe. On average, \textit{FlowTune} reduces the delay by 7\%. Therefore, \textit{FlowTune} achieves great delay improvements in both flows. The main difference is that while in VTR flow it could not benefit the \texttt{or1200}, in the OpenFPGA flow the \texttt{or1200} was greatly improved. Figure  \ref{fig:ofpga_tns} presents the OpenFPGA total negative slack results. We improved the baseline in 5 cases, up to 12\%. For one case, we had a 1\% TNS overhead. On average, we presented an average TNS reduction of ~5\%. Total negative slack has a similar trend in both, with gains when applying \textit{FlowTune}.

In conclusion, we can see that FlowTune framework with the domain-specific MAB algorithm can flexibly and effectively navigate flow optimizations in different logic synthesis DAG representations, and different PnR backends, and yet produce effective and consistent results. That positions \textit{FlowTune} as a versatile, light-weight, and portable flow exploration framework.

% {\color{red}Cunxi: think about the metrics that are interesting to report. e.g., Post-PnR timing, total neg slacks (TNS), wirelenghth, LUTs, routing congestion, etc.}

% \subsubsection{\yingjie{Yingjie: VTR 8.0 Post-PnR Evaluation:}}

% {{This part shows the post-routing evaluation results on area optimization, total routing wire cost, critical path delay and total slacks using VTR FPGA backend with and without FlowTune with six benchmarks, i.e., \texttt{bfly}, \texttt{dscg}, \texttt{fir}, \texttt{ode}, \texttt{or1200}, \texttt{syn2}. We also show the results with the same setup but with less FlowTune training efforts, configuring FlowTune by reducing the number of iteration of each stage while maintaining the number of stages, i.e., s:m is 2:10. 

% Overall, the performance for all four matrix, i.e., area, total wiring cost, critical path delay, and total slacks, can be improved significantly with FlowTune implemented for all designs except for design \texttt{or1200}. Specifically, 

% Figure \ref{fig:vtr_twl} shows the results of post-routing evaluation on total routing wirelength. The performance with FlowTune can be improved for all designs. Also, the results show that reduced FlowTune will lead to reduced optimization with some degradation. However, compared to the saved overhead, the performance of reduced FlowTune can be efficient. However, for design \texttt{or1200}, we can achieve few improvement results with FlowTune optimization.

% Figure \ref{fig:vtr_wns} shows the results of post-routing evaluation on critical path delay, i.e, the worst negative slacks. 

% Figure \ref{fig:vtr_tns} shows the results of post-routing evaluation on total negative in the design. The performance of all designs can be improved with full FlowTune implemented. For all four designs except for \texttt{or1200} and \texttt{fir}, the reduced FlowTune can perform better than the full FlowTune while for \texttt{or1200} and \texttt{fir}, the reduced FlowTune perform a little bit worse than the full FlowTune but still improve the performance compared to the original one.}}



 

% {\color{green}
% \subsubsection{OpenFPGA Post-PnR Evaluation}
% \textbf{Objectives for FlowTune:} the objective for FlowTune is to optimize area. We interface FlowTune with LSOracle for MIG optimization, and use OpenFPGA as backend for post-PnR evaluation. 
% We compare FlowTune against a high effort LSOracle recipe for MIG minimization that balances area and delay. Both the baseline and the FlowTune based recipes are based on resubsitution, rewriting, and refactoring, and apply the algebraic techniques depicted in \cite{} for MIGs manipulation. It does not include, however, the MIG Boolean optimizations. 


% The input for LSOracle is the benchmarks in BLIF format. The BLIF is read into a MIG network, and FlowTune is called to interface with LSOracle logic optimizer for MIG optimization. For FlowTune, we use $s:m$ = 2:30. Note that the we bound FlowTune to generate the flows with a similar length as the original high-effort LSOracle flow, so that the number of transformations are very similar. The recommended flow by FlowTune is then applied over the original network, and we dump it as a BLIF file to serve as input for the OpenFPGA backend flow.

% For prototyping the design, we use the OpenFPGA flow, creating a \textit{task} in OpenFPGA that takes as input the optimized design and a XML file describing a Stratix IV like architecture. To make sure the design can fit the architecture, we allow the auto-sizing feature, which runs a binary-search to find an architecture that can fit the design, and we then use the same size for prototyping the baseline and FlowTune optimized designs. Note that fine tuning the FPGA size could reveal more gains. All the results are collected post PnR within the OpenFPGA flow. Also, note that we \textit{skip} all the logic optimizations that usually take place in OpenFPGA, and just place and route the input design. 

% First, Figure  \ref{fig:lso_maxwl} presents the maximum WL for a net segment, for both the standard LSOracle flow as well as the FlowTune integration in LSOracle. We present up to 25\% reduction in the maximum WL, ....










 



%\section{Artifacts}











%\section{Conclusion}



==> results.tex <==
 
\section{Experimental Results}\label{sec:results}


